ORCAGen: Orchestrating Context-Aware Malware Deception with RAG-Guided Generative AI

Malware defenses often remove or isolate suspicious programs as quickly as possible. While effective for containment, this approach can also waste an opportunity to observe attacker behavior and deploy targeted countermeasures. ORCAGen takes a different approach: it uses GenAI to build malware-specific deception playbooks offline, validates them before deployment, and enforces only the verified logic at runtime. ORCAGen combines Retrieval-Augmented Generation (RAG) with structured prompt engineering to generate both proof-of-concept (PoC) malware and corresponding deception orchestration code. A curated knowledge base (KB) of malware procedures and active defense strategies grounds the generation process, helping the LLM produce threat-specific and executable deception logic rather than generic or hallucinated outputs. The generated PoC malware provides a safe and reproducible way to test whether a deception strategy can disrupt, redirect, or suppress targeted malware behavior before the strategy is added to the runtime playbook. We evaluate ORCAGen across GPT-4o, GPT-5.5, Gemini 3.5 Flash, Qwen3-Coder, and Claude Sonnet 4.5 using execution success, hallucination rate, refinement effort, deception effectiveness, and runtime overhead. The evaluation covers synthesized malware scenarios and 150 real-world malware samples across keyloggers, information stealers, and ransomware. Across the evaluated scenarios, GPT-5.5 required the fewest refinements and produced no observed hallucinated APIs, while Gemini 3.5 Flash achieved the lowest response time and runtime overhead. The results show that RAG-guided structured prompting can support the scalable construction of malware-specific deception playbooks that remain lightweight and deterministic during runtime enforcement.

==> IEEE-TPS/file-eval-old.tex <==
\section{Evaluation}\label{sec:evaluation}

%\subsection{Environment Setup}
This section evaluates ORCAGen across its two-phase workflow. First, we evaluate the offline generation and validation phase by measuring whether different LLMs can generate functional proof-of-concept (PoC) malware and corresponding deception orchestration code. Second, we evaluate the runtime enforcement phase by compiling validated orchestration logic into a deception playbook and measuring its effectiveness against synthesized and real-world malware samples. We evaluated five large language models: \textbf{GPT-4o, GPT-5.5, Gemini 3.5 Flash, Qwen3-Coder, and Claude Sonnet 4.5.} We accessed the GPT-4o and GPT-5.5 models via ChatGPT during the code generation process. Code generation was conducted on a Windows 11 Enterprise system equipped with a 13th Gen Intel(R) Core i7-13700 CPU (2.10 GHz), 32 GB RAM, and an NVIDIA GeForce RTX 3070 GPU. Both CPU and GPU resources were used to support stable performance during multi-step, token-intensive generation of PoC and orchestration code. All generated code was subsequently tested in a virtualized environment using VMware Workstation Pro 17. Each test case was executed on a Windows 7 virtual machine configured with a 13th Gen Intel(R) Core i7-13700 CPU (2.11 GHz) and 8 GB RAM. We selected Windows 7 because its lightweight execution environment reduces virtualization overhead and supports efficient testing of user-level Windows API interactions. While Windows 10 and Windows 11 introduce newer security features and system optimizations, the API-level behaviors used in our evaluation remain suitable for controlled validation in this testbed. This setup provides an isolated environment for safely executing PoC malware and evaluating deception effectiveness.


\subsection{Functionality Validation}
This subsection evaluates ORCAGen's offline generation and validation phase. The goal is to determine whether ORCAGen can generate technically valid PoC malware and corresponding deception orchestration code before adding the generated logic into the runtime playbook. The evaluation has two objectives: first, to determine whether the generated PoC malware executes the targeted malicious behavior; and second, to assess whether the generated orchestration code activates correctly and disrupts, redirects, or conceals that behavior in the controlled testbed.

\textbf{Setup:} We focus on three malware categories: keyloggers, information stealers, and ransomware. Each family exhibits distinct tactics, techniques, and procedures (TTPs) that shape its malicious behavior. For evaluation, we designed five simulation scenarios per family, totaling fifteen variants. In each case, ORCAGen was tasked with generating (i) a PoC malware sample that replicates a specific malicious behavior and (ii) corresponding orchestration code intended to disrupt, mislead, or neutralize that behavior. Both the PoC and orchestration code were executed in a controlled virtual environment during offline validation. Execution traces, including keystroke logs, clipboard captures, file scanning attempts, and encryption attempts, were monitored to confirm that the PoC reproduced the intended malicious activity. The generated orchestration code was then evaluated by observing whether it successfully intervened and achieved its defensive goal without revealing the presence of countermeasures. A complete list of the simulation scenarios used for each malware category is available in our GitHub repository~\cite{orcagen}.


\textbf{Evaluation Metrics:} We report two primary metrics. First, \textbf{PoC execution rate} measures the percentage of generated PoCs that executed without errors and reproduced the expected malicious behavior. Second, \textbf{orchestration code execution rate} measures the percentage of generated orchestration instances that executed successfully and disrupted or misdirected the PoC malware during validation. Results were recorded under three conditions: \textbf{zero-shot execution}, where the generated code worked on the first attempt; \textbf{minor corrections}, where the code required straightforward fixes before execution; and \textbf{major reliability issues}, where the output contained structural or semantic flaws. Minor corrections included missing library imports, character encoding mismatches (ANSI/Unicode), C++ compatibility adjustments, and simple type-casting errors. Major reliability issues were defined as hallucinations, such as non-existent APIs, fabricated system calls, or logically impossible code.


\textbf{Results and Discussion:}
Figure~\ref{fig:functionality_validation} shows the ability of each GenAI model to generate functional PoC malware and corresponding orchestration code across keyloggers, information stealers, and ransomware. GPT-4o achieved a 100\% PoC execution rate for keyloggers and ransomware, with only one minor correction required for information stealers. Its orchestration code executed successfully in 66.67\% of cases (10/15), while the remaining 33.33\% (5/15) required minor corrections. GPT-5.5 delivered the strongest overall performance. It achieved 93.33\% successful PoC execution (14/15), with only 6.67\% requiring minor correction (1/15). Its orchestration code achieved 100\% zero-shot execution across all three malware categories. Gemini 3.5 Flash showed variable performance for PoC generation. It achieved 100\% zero-shot PoC execution success for keyloggers, but its performance for information stealers and ransomware dropped to 60\% (3/5), with 40\% (2/5) requiring modifications. Overall, its PoC execution success was 73.33\%. For orchestration code, Gemini achieved 100\% zero-shot execution across keyloggers, information stealers, and ransomware. Qwen3-Coder also showed mixed results. For PoC execution, it achieved 60\% success for keyloggers, 100\% success for information stealers, and 80\% success for ransomware. However, its orchestration code required more refinement. It achieved 40\% zero-shot success for both keyloggers and information stealers, with the remaining 60\% requiring further prompt refinements. For ransomware, none of the orchestration outputs executed successfully in zero-shot form, and all required additional refinement before successful execution. Due to strict privacy and content safety policies, Claude Sonnet 4.5 did not generate PoC malware code. Therefore, we evaluated Claude Sonnet 4.5 only for orchestration code generation using PoCs generated by GPT-5.5. Claude achieved 80\% orchestration execution success for keyloggers and information stealers, with 20\% requiring correction. For ransomware, it achieved 20\% success, while 80\% required refinement. Table~\ref{tab:error_categories} summarizes common error types across models. GPT-4o, GPT-5.5, Gemini 3.5 Flash, and Claude Sonnet 4.5 exhibited limited issues, mostly related to encoding mismatches and minor compatibility fixes. Qwen3-Coder faced broader issues, including hallucinated APIs, missing headers, type-casting errors, and compatibility mismatches.

Overall, these findings show that the evaluated LLMs can generate operational PoC and orchestration code, but they differ substantially in the amount of refinement required before validation. \textbf{GPT-5.5} delivered the strongest balance across PoC generation and orchestration code generation, with high execution success, minimal correction effort, and no observed hallucinated APIs. In contrast, Qwen3-Coder required more post-processing, highlighting the importance of structured prompting, retrieval grounding, and validation before adding generated deception logic to the runtime playbook.

\begin{table}[h]
\caption{Common Error Types in Generated Code Across GenAI Models}
\vspace{-0.3cm}
\centering
\renewcommand{\arraystretch}{1.2} % Adjust row height
\setlength{\tabcolsep}{4pt} % Adjust column width
\scriptsize % Reduce font size
%\begin{tabular}{|l|c|c|c|c|}
\begin{tabular}{|p{1.9cm}|p{0.8cm}|p{1.1cm}|p{1.2cm}|p{0.9cm}|p{1.3cm}|}
\hline
\textbf{GenAI Model} & \textbf{Missing Header Files} & \textbf{Character Encoding Mismatch} & \textbf{C++ Compatibility Issues} & \textbf{Type Casting Errors} & \textbf{Hallucinated APIs/Data} \\ \hline
GPT-4o & 1 & 5 & 0 & 0 & 0 \\ \hline
GPT-5.5 & 0 & 0 & 1 & 0 & 0 \\ \hline
Gemini 3.5 Flash & 1 & 0 & 2 & 1 & 0 \\ \hline
Qwen3-Coder	& 8 & 3 & 1 & 1 & 3 \\ \hline
Claude Sonnet 4.5 & 3 & 0 & 1 & 1 & 0 \\ \hline
\end{tabular}
\label{tab:error_categories}
\end{table}

\subsection{Orchestration Accuracy}

\subsubsection{Against Synthesized Malware Samples}
This subsection evaluates the consistency and reliability of orchestration code generated by ORCAGen in deceiving or neutralizing the behavior of its corresponding PoC malware, without disrupting legitimate system functionality. The evaluation covers three malware families including keyloggers, information stealers, and ransomware with five simulation scenarios per family, totaling 15 test cases. For each case, ORCAGen generates PoC malware and deception orchestration code, which are deployed in a controlled virtual environment. The success of each orchestration is measured by its ability to suppress or mislead the behavior of the targeted malware at runtime.

The primary metric is the \textbf{deception success rate}, which measures the percentage of executions in which the orchestration code successfully altered, blocked, or redirected the malicious activity. As introduced earlier (Section~\ref{prompt_egnr}), we also tracked the number of \textbf{prompt refinements} required for each model to reach perfect success. To further assess reliability, we measured two failure conditions: \textbf{false positives}, where legitimate processes were unintentionally disrupted, and \textbf{false negatives}, where the orchestration failed to intervene and allowed the malware to complete its behavior. Together, these metrics provide a comprehensive view of ORCAGen’s robustness in real-time deception.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\columnwidth]{images/deception_success_rate.pdf}
    \vspace{-0.7cm}
    \caption{Orchestration Accuracy of GenAI Models.}
    \vspace{-0.2cm}
    \label{fig:orchestration_accuracy}
\end{figure}

\textbf{Results and Discussion:} 
Figure~\ref{fig:orchestration_accuracy} shows the orchestration accuracy across evaluated models. GPT-4o, GPT-5.5, Gemini 3.5 Flash, Qwen3-Coder, and Claude Sonnet 4.5 all eventually achieved a perfect deception success rate of 100\% which indicates that the generated orchestration code effectively disrupted the behavior of the PoC malware effectively. However, a closer examination of the results with respect to zero-shot performance (i.e., without any prompt refinement) reveals more variation. GPT-5.5 and Gemini 3.5 Flash achieved 100\% zero-shot effectiveness, successfully executing orchestration code without any refinement across all evaluated cases. GPT-4o followed closely by achieving zero-shot effectiveness of 66.67\% (10/15 cases), while Claude Sonnet 4.5 achieved 60\% (9/15 cases) and Qwen3-Coder achieved 26.67\% (4/15 cases). As prompt refinements were introduced, success rates improved gradually. GPT-5.5 and Gemini 3.5 Flash already maintained 100\% success without requiring additional refinement. GPT-4o and Claude Sonnet 4.5 achieved 100\% success after just two average refinements, while Qwen required three average refinements to reach 100\% deception success rate, reflecting a greater dependency on iterative guidance. This result highlights the importance of model selection and prompt engineering when aiming for reduced post-processing effort and low-overhead of fully automated deception systems. Additionally, these models showed no instances of false positives or false negatives, confirming both the precision and safety of their deception strategies. The absence of false positives demonstrates that legitimate system processes remained unaffected, while the lack of false negatives reflects consistent success in altering or neutralizing the targeted malicious behavior. These results support ORCAGen’s reliability in producing technically accurate and operationally sound defensive interventions across multiple LLMs.

\textbf{Ethics and Safety:} ORCAGen generates PoC malware only for controlled validation of deception logic. All PoCs were behavior-limited and executed in isolated virtual machines. Ransomware PoCs operated only on dummy files, credential theft was redirected to synthetic artifacts, and network exfiltration was disabled or redirected to local sinks. We do not release weaponizable malware code; released artifacts include sanitized prompts, KB schemas, benign harnesses, and evaluation metadata.

% We restricted the maximum number of refinements to three, and Claude Sonnet was unable to reach 100\% success within this limit. 

\subsubsection{Against Real-World Malware Samples}
To assess whether ORCAGen's generated deception playbooks remain effective beyond synthesized PoC malware, we evaluated them against 150 real-world malware samples collected from publicly available repositories. The dataset includes 50 samples from each malware family considered in this study: keyloggers, information stealers, and ransomware. These samples cover multiple subfamilies within each category; the complete subfamily list and per-sample evaluation details are provided in our anonymous repository~\cite{orcagen}. Each sample was executed in a controlled and instrumented environment, and the corresponding pre-generated deception playbook was deployed to determine whether it could alter, suppress, or safely redirect the malware's intended behavior.

For information stealers, ORCAGen protected credential-access targets commonly abused by malware, including browser credential stores, FTP credentials, and application-specific credential files such as those used by email clients. Following the target categories identified in prior work~\cite{sajid2020dodgetron}, ORCAGen monitored file operations on these sensitive targets and checked whether the accessing process was absent from a predefined whitelist of legitimate applications. When both conditions were satisfied, the process was treated as suspicious and redirected to pre-generated honey credential files instead of real credential artifacts.

For ransomware, ORCAGen used two complementary deception strategies inspired by prior bait-based ransomware defenses~\cite{sajid2025randecepter}. First, bait files were exposed through soft links at the top and bottom of monitored directories to reduce storage overhead while preserving coverage. If a bait file was encrypted, ORCAGen identified the responsible process and marked it as ransomware when the process was not part of the trusted whitelist. Second, ORCAGen monitored destructive file operations, including deletion and overwrite attempts, and returned deceptive success or failure responses while preserving the original files. These interventions were applied only to selected high-value user locations and excluded temporary folders or other low-value directories where benign applications frequently perform high-volume file modifications.

For keyloggers, ORCAGen focused on input, clipboard, and screen-capture behaviors. It monitored suspicious attempts to capture keyboard input, access clipboard content, or collect screen and cursor information. For keyboard and clipboard logging, ORCAGen suppressed or replaced captured content with decoy input or honey clipboard data. For screen logging, it redirected capture attempts toward decoy visual information, preventing the malware from observing the actual user screen state. These interventions were applied only to suspicious processes to avoid disrupting benign applications that legitimately use input, clipboard, or screen-capture functionality.

Table~\ref{tab:real_malware_accuracy} summarizes the outcomes. We classify each execution into three categories: \textbf{complete neutralization}, where the malware's intended behavior was fully disrupted or redirected; \textbf{partial disruption}, where only part of the malicious behavior was affected or observable; and \textbf{deception failure}, where the playbook produced no observable defensive effect.

\begin{table}[h]
\caption{ORCAGen Orchestration Accuracy against Real-World Malware}
\vspace{-0.3cm}
\centering
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{4pt}
\scriptsize
\begin{tabular}{|p{2.0cm}|p{1.8cm}|p{1.5cm}|p{1.5cm}|}
\hline
\textbf{Malware Family} & \textbf{Complete Neutralization} & \textbf{Partial Disruption} & \textbf{Deception Failure} \\ \hline
Keylogger & 92\% & 0\% & 8\% \\ \hline
Information Stealer & 100\% & 0\% & 0\% \\ \hline
Ransomware & 96\% & 2\% & 2\% \\ \hline
\end{tabular}
\vspace{-0.3cm}
\label{tab:real_malware_accuracy}
\end{table}

\textbf{Results and Discussion:}
ORCAGen achieved strong effectiveness across all three real-world malware families. For keyloggers, it completely neutralized 92\% of samples, while 8\% were not successfully deceived. The four failed samples used direct keyboard-state polling combined with internal key mapping; ORCAGen could suppress or simulate key-state responses, but it could not consistently replace the malware's internally reconstructed key values with decoy keystrokes. For information stealers, ORCAGen achieved 100\% complete neutralization by redirecting unauthorized credential-access attempts to honey credential artifacts. For ransomware, ORCAGen completely neutralized 96\% of samples, partially disrupted 2\%, and failed against 2\%. The partially disrupted case involved a ransomware sample that depended on a C\&C server to download an additional component. Because the C\&C infrastructure was unavailable during testing, only part of the ransomware behavior could be observed, so we conservatively classified the outcome as partial disruption. Overall, these results suggest that ORCAGen's playbooks can transfer from synthesized PoC validation to real-world malware samples when the malicious behavior interacts with monitored input, credential, file-system, or API-level targets.

% \subsubsection{Against Real-World Malware Samples}
% To extend the evaluation, we tested ORCAGen against 50 real-world malware samples spanning keyloggers, information stealers, and ransomware. For each family, we designed three representative deception scenarios. For example, in the case of information stealers targeting browser-stored credentials, the orchestration was tasked with injecting fake credentials to mislead the malware. This resulted in a total of 150 execution trials (50 malware samples $\times$ 3 scenarios each).

% Compared to the synthesized PoCs, this evaluation posed greater challenges because the LLMs did not have access to the exact implementation details of the malware. Instead, deception strategies were inferred from abstract behavior descriptions and malware analysis reports. As expected, this increased the average number of \textbf{prompt refinements} required to achieve functional orchestration. Nevertheless, the models consistently achieved 100\% deception success within five refinements.

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.95\columnwidth]
%     {images/real_malware_accuracy.pdf}
%     \vspace{-0.1cm}
%     \caption{ORCAGen Orchestration Accuracy against Real World Malware.}
%     \vspace{-0.3cm}
%     \label{fig:real_malware_accuracy}
% \end{figure}

% \textbf{Results and Discussion:} 
% Figure~\ref{fig:real_malware_accuracy} presents the orchestration accuracy across ChatGPT-4.1, ChatGPT-4o, and Gemini 2.5 Flash. ChatGPT-4.1 again demonstrated the strongest zero-shot performance, successfully deceiving 60\% of cases (90/150), followed by ChatGPT-4o at 53.33\% (80/150) and Gemini at 40\% (60/150). With successive refinements, performance steadily improved: ChatGPT-4.1 reached 93.33\% success by the second refinement and 98.67\% by the third, while ChatGPT-4o required up to four refinements to exceed 98\%. Gemini, though more dependent on iterative refinements, rose from 40\% at zero-shot to 96\% by the fourth refinement and achieved perfect accuracy after the fifth. Notably, across all 150 executions, no false positives were recorded, ensuring legitimate processes remained unaffected. Similarly, no false negatives were observed once orchestrations were refined to functional states. While refinement demands were higher than in the synthetic PoC cases, the results confirm ORCAGen’s robustness and adaptability in handling real-world malware families. These findings underscore the value of retrieval-augmented deception strategies, which enable accurate defensive responses even when relying on higher-level malware analysis reports rather than source code.

\subsection{Ablation Study on Prompting Strategies}
We compare three prompting strategies for generating orchestration code: \textbf{Direct Prompting}, \textbf{RAG-Enhanced Prompting}, and \textbf{ORCAGen}. In \textbf{Direct Prompting}, the LLM receives only a direct instruction to generate deception code without any external contextual support. \textbf{RAG-Enhanced Prompting} extends direct prompting by including the deception strategy retrieved from the knowledge base through retrieval-augmented generation (RAG) to provide contextual guidance during code generation. In contrast, \textbf{ORCAGen} combines retrieved deception strategy through RAG with a structured prompt engineering approach to generate operational deception code. The prompt engineering approach explicitly specifies the objective, contextual information, expected output format, and relevant examples to guide the model toward producing technically valid and operational deception code. We conducted the ablation study using the same 15 scenarios used in the functionality validation phase to ensure experimental consistency and comparability. Furthermore, we adopted the same prompt refinement procedure used during functionality validation phase, where iterative prompt modifications were applied until functional orchestration code was successfully generated or reached a maximum of five attempts. To evaluate effectiveness, we measured the deception success rate across increasing numbers of prompt refinements, representing the average number of iterative prompt modifications required to achieve functional orchestration code. Figure~\ref{fig:prompting_strategy_comparison} presents the impact of prompt refinement on deception success rate across the three prompting strategies, with all evaluations conducted using the GPT-5.5 model.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\columnwidth]{images/prompting_strategy.pdf}
    \caption{Ablation Study Comparing Different Prompting Strategies.}
    \label{fig:prompting_strategy_comparison}
\end{figure}

\textbf{Results and Discussion:}
Direct Prompting achieved 0\% deception success in zero-shot execution. It improved gradually with refinement and reached 13.33\% after two refinements and 46.67\% after five. This result suggests that prompt iteration alone is insufficient to consistently generate reliable deception orchestration. When RAG was introduced, RAG-Enhanced Prompting showed stronger results. The deception success rate increased to 53.33\% after only one average refinement and improved to 73.33\% after two average refinements. However, no additional improvement was observed beyond this point, with performance remaining constant through five refinements. This shows that integrating deception strategy through external knowledge sources significantly improves the model’s ability to generate operational deception orchestration code, but still fails to consistently achieve full success. In contrast, ORCAGen achieved the strongest overall performance, reaching a 100\% deception success rate in zero-shot execution, without requiring any prompt refinement. This indicates that the integration of RAG with structured prompt engineering enables ORCAGen to consistently produce functional deception orchestration code on the first attempt.

Overall, these findings show that while retrieval augmentation improves deception generation compared to direct prompting, ORCAGen significantly outperforms both baselines by achieving perfect deception success in zero-shot execution. The results highlight the importance of combining RAG with structured prompting, rather than relying solely on iterative prompt refinement.



\subsection{Performance Measurement}
To evaluate the effectiveness and efficiency of GenAI models during the offline generation phase of ORCAGen, performance was quantified using four key evaluation metrics: prompt refinements, hallucination rate, runtime overhead, and response time. These metrics were used to assess the ability of GPT-4o, GPT-5.5, Gemini 3.5 Flash, Qwen3-Coder, and Claude Sonnet 4.5 to generate technically valid and operational code for both malware proof-of-concepts (PoCs) and their corresponding orchestration logic. For each scenario, ORCAGen generated PoC malware and deception orchestration code using structured prompts, and the resulting outputs were systematically evaluated for completeness, correctness, and run-time reliability.

\begin{table}[h]
\caption{Performance of ORCAGen across different GenAI Models}
\vspace{-0.3cm}
\centering
\renewcommand{\arraystretch}{1.3} % Adjust row height
\setlength{\tabcolsep}{4pt} % Adjust column width
\scriptsize % Reduce font size
%\begin{tabular}{|l|c|c|c|c|}
\begin{tabular}{|p{1.9cm}|p{1.8cm}|p{1.4cm}|p{1.0cm}|p{1.0cm}|}
\hline
\textbf{GenAI Model} & \textbf{Prompt Refinements (Avg)} & \textbf{Hallucination Rate (Avg)} & \textbf{Overhead (ms)} & \textbf{Response Time (s)} \\ \hline
GPT-4o & 0.47 & 0 & 84.35 & 71.4 \\ \hline
GPT-5.5 & 0.07 & 0 & 27.69 & 54.21 \\ \hline
Gemini 3.5 Flash & 0.27 & 0 & 18.32 & 34.92 \\ \hline
Qwen3-Coder & 1.73 & 0.27 & 183.56 & 71.32 \\ \hline
Claude Sonnet 4.5 & 0.53 & 0 & 122.68 & 74.5 \\ \hline
\end{tabular}
\vspace{-0.3cm}
\label{tab:performance_genai}
\end{table}

Each code generation session was tracked to measure the number of \textbf{prompt refinements (regenerations)} required to achieve functional outputs. Following generation, all code was manually reviewed to identify instances of \textbf{hallucinated APIs} or \textbf{function calls}, including non-existent, misused, or syntactically invalid elements. Once validated as operational, orchestration code was injected into the malware process within a virtual machine to measure \textbf{runtime overhead}, defined as the additional execution latency introduced by the orchestration DLL. Overhead was averaged across ten independent trials to ensure statistical consistency. Finally, we measured \textbf{response time}, defined as the end-to-end latency for each model to generate both the PoC malware and the corresponding deception orchestration code.


\textbf{Results and Discussion:} 
Table~\ref{tab:performance_genai} presents the comparative performance of ORCAGen across the evaluated GenAI models using four operational metrics. GPT-4o demonstrated reliable consistency, requiring an average of only 0.47 refinements per task and exhibiting no hallucinated outputs. Its runtime overhead was moderate (84.35 ms), although its response time was relatively slow (71.4 seconds), indicating a trade-off between reliability and generation latency. GPT-5.5 demonstrated the strongest overall balance between efficiency and reliability. It required the lowest number of refinements (0.07 on average), exhibited no hallucinations, and maintained a low runtime overhead of 27.69 ms. Its average response time (54.21 seconds) remained within operational limits. Gemini 3.5 Flash outperformed other models in responsiveness, achieving the fastest average response time (34.92 seconds) with the lowest runtime overhead (18.32 ms). It also required only 0.27 average prompt refinements and produced no hallucinated outputs,  suggesting a strong balance between accuracy and efficiency. Claude Sonnet 4.5 maintained strong generation quality with 0 hallucinations and required 0.53 average refinements. However, its runtime overhead was relatively high (122.68 ms), and response time was the slowest among all models (74.5 seconds). Qwen3-Coder exhibited more variability, achieving the highest runtime overhead among all evaluated models (183.56 ms), and the second highest response time of 71.32 seconds. The model required the highest number of refinements (1.73 on average) and exhibited a hallucination rate of 0.27. These findings indicate a greater reliance on iterative corrections to produce functional outputs, reflecting weaknesses in both structural and semantic accuracy. 

\textbf{Overall Analysis:} The results indicate that all evaluated GenAI models are capable of producing technically valid and deployable outputs, but with varying trade-offs between reliability and responsiveness. GPT-5.5 is most suitable for rapid playbook construction because it required the fewest refinements and produced no hallucinated APIs, while Gemini 3.5 Flash produced the lowest measured runtime overhead among the evaluated orchestration outputs. In contrast, Qwen’s higher refinement demand and hallucination rate highlight the importance of improved prompt engineering or post-processing for sustained operational use.

\subsection{Performance Comparison with SPADE}
This section presents a comparative evaluation of our proposed ORCAGen framework against SPADE \cite{ahmed2025spade}, a GenAI-driven system that generates adaptive deception ploys through structured prompt engineering. SPADE automates the creation of artifacts such as honeyfiles, patches, and API hooks using carefully designed prompts. However, it does not incorporate functionality validation of the generated deception logic, nor does it support runtime orchestration against malware behavior. Importantly, SPADE does not include the generation of malware proof-of-concepts (PoCs), which limits its ability to test deception artifacts against realistic adversarial behaviors. To enable a direct comparison, we reproduced 14 representative scenarios from the SPADE evaluation and applied both the SPADE prompting strategy and our ORCAGen framework. For evaluation, we measured the \textbf{deception success rate} across increasing numbers of prompt refinements, defined as the average number of iterative adjustments required to generate functional deception logic - which is deployable against synthesized PoC malware. Figure~\ref{fig:spade_vs_orcagen} reports results for ChatGPT-4o, ChatGPT-4.1, and Gemini 2.5 Flash across both frameworks.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\columnwidth]
    {images/spade_vs_orcagen.pdf}
    \vspace{-0.5cm}
    \caption{Performance Comparison between SPADE and ORCAGen.}
    \vspace{-0.3cm}
    \label{fig:spade_vs_orcagen}
\end{figure}

\textbf{Results and Discussion:} ORCAGen consistently outperformed SPADE across all models and refinement thresholds. For GPT-4o, SPADE achieved only 7.14\% success rate (1/14 case) by the fifth average refinement and reached at 50\% success rate (7/14 cases) after ten average refinements. In contrast, ORCAGen achieved 21.42\% deception success rate (3/14 cases) even at zero-shot, 64.29\% (9/14 cases) after one average refinement, and reached 100\% success rate (14/14 cases) by the fifth average refinement. For GPT-4.1, ORCAGen reached 71.43\% success (10/14 cases) with no refinements, achieving full deception success after only one average refinement. SPADE only reached 42.86\% deception success rate (9/14 cases) even after eight average refinements, and remained below 65\% (9/14 cases) even after ten average refinements. For Gemini 2.5 Flash, SPADE failed to produce any successful deception across all refinement levels. However, ORCAGen demonstrated steady improvements. It showed gradual improvement, from 28.57\% (4/14 cases) at zero-shot to full 100\% (14/14 cases) deception success rate by the fifth average refinements.

These results highlight the role of retrieval-augmented generation (RAG) in enhancing both zero-shot effectiveness and refinement efficiency. Unlike SPADE, which relies solely on structured prompting, ORCAGen integrates prompts with curated, threat-relevant knowledge such as malware-specific techniques and associated countermeasures. This significantly improves zero-shot performance and reduces the number of prompt iterations required to generate functional and deployable deception ploys. Moreover, ORCAGen incorporates functionality validation by testing the generated orchestration code against active PoC malware in runtime environments, ensuring that outputs are not only syntactically correct but also functionally effective. While SPADE's focus on automating the generation of deception artifacts through structured prompting represents an important step forward, its lack of runtime validation limits its assurance in real-world settings.

==> IEEE-TPS/file-methodology-old.tex <==
\section{ORCAGen: System Overview}\label{sec:methodology}
\subsection{System Architecture}
ORCAGen is a GenAI-driven framework for constructing malware-specific deception playbooks in post-compromise scenarios. Rather than relying on static, manually engineered ploys, ORCAGen integrates Retrieval Augmented Generation (RAG) with structured prompts to produce both proof-of-concept (PoC) malware and corresponding deception orchestration code during offline playbook construction. The generated logic is validated in a controlled environment, and only verified deception strategies are compiled into a Super DLL for runtime enforcement. Figure~\ref{fig:system_architecture} illustrates the end-to-end workflow, from knowledge acquisition to validation of deception strategies.


The process begins with the selection of a target malware type (e.g., keyloggers, information stealers, or ransomware). Relevant threat intelligence is then collected from academic publications, malware blogs, incident reports, and security forums, and organized into two structured knowledge bases. The first knowledge base captures malware procedures, including entries for malware family, attack technique, and detailed behavioral descriptions. The second knowledge base captures active defense strategies, mapping each malware family and technique to its corresponding deception strategy. Together, these knowledge bases serve as the retrieval layer for RAG, with the implementation details described in Section~\ref{rag_impl}. It provides context-specific intelligence that directly informs the generation of two components: (i) proof-of-concept (PoC) malware and (ii) corresponding deception orchestration code. Both components are produced using structured prompts that define objectives, expected outputs, contextual information, and examples. In the final stage, the generated PoC malware is executed in a controlled environment, and the associated orchestration logic is deployed to evaluate its effectiveness in disrupting or misleading malicious behaviors. Only verified deception logic is compiled into the validated playbook, which is then used during runtime enforcement. The following sections describe each stage of this workflow in detail.

\subsection{Knowledge Base Creation for RAG}\label{kb}


We construct two structured knowledge bases (KBs) where one captures malware behaviors and another one maps those behaviors to corresponding deception strategies. In this work, we focus primarily on keyloggers, information stealers, and ransomware, chosen because their behaviors involve clear and observable system interactions such as keystroke capture, credential theft, and file encryption. These behaviors provide an ideal starting point for simulating adversarial actions and evaluating deception effectiveness. However, the framework itself is designed to generalize and can be extended to other malware variants.



\begin{table*}
\caption{Example of Knowledge Base}
\centering
\renewcommand{\arraystretch}{1.3} % Adjust row height
\setlength{\tabcolsep}{4pt} % Adjust column width
\footnotesize % Reduce font size
\begin{tabular}{|p{1.4cm}|p{1.3cm}|p{6.2cm}|p{8.1cm}|}
\hline
\textbf{Malware Family} & \textbf{Attack Technique} & \textbf{Behavioral Description} & \textbf{Deception Strategy} \\ \hline

Information Stealer & File System Scanning & Recursively scans directories and locates sensitive files based on target extensions and filenames (e.g., .json, .conf, .ini, .txt, api\_key, browser profiles, wallet.dat). Uses Windows APIs such as \texttt{FindFirstFile}, \texttt{FindNextFile} to scan files in directories (e.g., \verb|C:\\Users\\*\\Documents|) and return the filenames. & \textbf{Filesystem API Hooking:} Intercept calls to file system scanning and access APIs such as \texttt{FindFirstFile, FindNextFile, CreateFile, ReadFile}, etc. Return decoy filenames instead of the actual search results to mislead malware. \\ \hline

Keylogger & Screen Logging & Periodically takes screenshots or captures the display screen when certain events occur. Screen capture APIs (e.g., \texttt{BitBlt, PrintWindow}) captures screen content. & \textbf{Screen Capture Prevention:} The screen capture APIs (e.g., \texttt{BitBlt, PrintWindow}) captures screen content. Intercept screenshot capture APIs and replace captured images with decoy screenshots. For example, hook the \texttt{BitBlt} and \texttt{PrintWindow} APIs to inject decoy images. Ensure legitimate screen capture requests remain functional. \\ \hline

Ransomware & File-Based Encryption & Targets specific file extensions (e.g., .docx, .xlsx, .db, .txt) while skipping critical operating system and application files to keep the system functional. Uses filters or hardcoded lists of extensions to select files for encryption in a specific directory (\verb|C:\\Users\\*\\Documents|). Employs Windows APIs like \texttt{FindFirstFile} and \texttt{FindNextFile} to enumerate files, and \texttt{CreateFile, ReadFile, WriteFile} to read and overwrite file contents with encrypted data. & \textbf{File I/O Hooking:} Intercept file operation APIs such as \texttt{CreateFile, WriteFile, SetFilePointer, FlushFileBuffers} to detect or modify ransomware behavior. Check for suspicious access to large numbers of documents. The goal is to implement a FakeFailure/FakeSuccess approach for specific file types where the ransomware receives error messages, indicating failed to encrypt files (FakeFailure), or the ransomware perceives the encryption as complete and receive a fake success message while no actual file is encrypted (FakeSuccess) while legitimate file operations remain functional. \\ \hline

\end{tabular}
\label{tab:kb_example}
% \vspace{-0.5cm}
\end{table*}



To populate the KBs, we designed a systematic collection pipeline that combines both lexical and semantic search. Exact-phrase queries (e.g., ``GetAsyncKeyState keylogger'') were used to retrieve documents with precise technical discussions, while flexible multi-term queries (e.g., \texttt{GetAsyncKeyState + keylogging + evasion}) ensured inclusion of sources where relevant terms appear in different contexts or orders. We seeded our searches with MITRE ATT\&CK techniques such as \texttt{T1056: Input Capture}, \texttt{T1003: Credential Dumping}, and \texttt{T1486: Data Encrypted for Impact}, and extended them with deception-specific modifiers including ``API hooking mitigation,'' ``clipboard decoy,'' and ``fake credential injection.'' To maximize coverage, two complementary pipelines were used: (i) a custom web crawler that systematically collected documents from academic research, threat intelligence reports, malware blogs, and security forums, and (ii) Perplexity AI’s semantic search engine to capture contextually relevant but lexically diverse sources. Documents appearing consistently across both pipelines were prioritized as they indicated higher topical reliability. Retrieved texts were stored locally for manual validation and structured processing.



From this corpus, we extracted structured entries consisting of four key elements: (i) malware family, (ii) attack techniques, (iii) behavioral description, and (iv) deception strategies. Importantly, deception strategies were encoded at two levels of abstraction. At the fine-grained level, we captured technical details such as system calls and API usage (e.g., \texttt{GetAsyncKeyState}, \texttt{SetWindowsHookEx}, or registry modifications). At the higher level, we included generic deception ploys such as injecting false keystrokes, creating decoy credentials, or deploying fake file structures. This layered representation enables ORCAGen to generate proof-of-concept malware using precise API-level details while also producing orchestration code that generalizes across multiple adversarial behaviors. We stored information such as malware family, attack procedures/techniques, and behavioral description in the first knowledge base named Malware Procedures. In the second knowledge base named Active Defenses, we stored information such as attack procedures/techniques and corresponding deception strategies. The final knowledge bases are encoded in a structured JSON format to facilitate seamless integration with the RAG pipeline. Figure~\ref{fig:kb_creation} shows the KB construction workflow, and Table~\ref{tab:kb_example} provides representative entries.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=.95\columnwidth]{images/KB_creation.pdf}
    \vspace{-0.3cm}
    \caption{Knowledge Base Creation Process.}
    \label{fig:kb_creation}
    \vspace{-0.2cm}
\end{figure}

% The final KB is encoded in a JSON schema segmented by malware family, technique, and deception strategy for seamless integration into the RAG pipeline. Figure~\ref{fig:kb_creation} shows the KB construction workflow, and Table~\ref{tab:kb_example} provides representative entries.

\subsection{RAG Implementation}\label{rag_impl}

The Retrieval-Augmented Generation (RAG) component supplies task-specific malware and defense knowledge during offline playbook construction. Rather than exposing the entire knowledge base (KB) to the model, ORCAGen retrieves relevant entries for each generation task and injects them into the \emph{Context} component of the prompt template described in Section~\ref{prompt_egnr}. The KB is stored as structured entries: malware procedure entries capture malware family, attack technique, behavioral description, relevant APIs or artifacts, affected resources, and execution patterns, while active defense entries capture deception objectives, intervention points, required hooks or monitors, expected responses, and safety constraints. %Together, these entries cover the malware families evaluated in this study, including keyloggers, information stealers, and ransomware, along with their associated API-level and file-system behaviors.
In the current prototype, the KB contains \textbf{8} malware procedure entries and \textbf{19} active defense entries covering \textbf{3} malware families, \textbf{8} attack techniques, and \textbf{28} API-level or file-system indicators.
% \textcolor{red}{Shihab can you fill in these numbers from the RAG KB you have used? - if you can't quantify these numbers then just remove this comment+last line and un-comment the second last line.}


ORCAGen currently supports two RAG modes. For cloud-hosted LLMs, including ChatGPT, Gemini, and Claude, we used the platforms' built-in knowledge or file-grounding mechanisms to make the KB available during generation. For local models, such as Qwen through Ollama and Open WebUI, we used an external lightweight RAG pipeline that indexes the structured KB, forms queries from the malware family, target behavior, attack technique, and generation objective, and retrieves the top-\textbf{k} relevant entries for prompt injection. For PoC generation, retrieved entries describe the malware behavior, relevant APIs, and expected execution pattern. For orchestration generation, retrieved entries describe the corresponding active defense strategy and are combined with the generated PoC code. Across both modes, ORCAGen follows the same high-level workflow: query the KB for relevant threat and defense entries, inject the retrieved context into the structured prompt, and generate either PoC malware or deception orchestration code. This hybrid setup allows ORCAGen to operate across both cloud-hosted and local LLM backends, but it also introduces a reproducibility limitation because cloud platforms do not expose full control over their internal retrieval mechanisms. Because cloud-hosted models rely on provider-managed retrieval, our cross-model results should be interpreted as a comparison of practical LLM-backend configurations rather than a controlled comparison of model weights alone. To address this, our planned deployment uses a unified external RAG layer for all LLMs: ORCAGen performs retrieval externally, logs the query and retrieved KB entries, constructs the final prompt, and sends it to online models through API-token-based invocation. In this design, only the communication interface changes from browser-based interaction to API-based communication, while the retrieval and prompt-construction pipeline remains consistent across local and cloud-hosted models.


\subsection{Prompt Engineering}\label{prompt_egnr}
Prompt engineering is very important to adapting general-purpose large language models (LLMs) for specialized cybersecurity tasks. Within ORCAGen, prompt templates serve as structured instructions that guide the model to generate malware-specific outputs, from proof-of-concept (PoC) code to orchestration-level defenses. Each template embeds operational context, technical constraints, and expected output structure, ensuring that the generated content is precise, reproducible, and directly deployable into deception systems.


\begin{figure*}[!ht]
    \centering
    \includegraphics[width=.99\textwidth] {images/PromptDesign.pdf}
    \vspace{-0.3cm}
    \caption{Formal Prompt Structure.}
    \vspace{-0.3cm}
    \label{fig:prompt_structure}
\end{figure*}
\textbf{Initial Prompt:} To ensure consistency and functionality in LLM outputs, we used an initial prompt that guides the generation of both PoC malware and corresponding orchestration code. This prompt provides a base project structure that contains three key components: a PoC malware sample, a DLL-based API hooking module, and an injector for deploying the DLL into a target process. By providing this structured template along with partial code snippets, we guide the LLM with a clear understanding of the expected format and execution flow. Such guidance significantly improves generation quality. Without it, LLMs often produce outputs of incomplete structure, mismatched function signatures or non-functional code. Providing an existing project structure ensures the outputs are executable, testable and aligned with the intended workflow.

\textbf{Core Components of the Prompt Template:} To enable consistent and targeted generation, the prompt template is structured into four components: objective/task, output format, context, and example. Each element is designed to capture a distinct aspect of the generation process, forming a modular template structure that allows flexibility and customization. Figure~\ref{fig:prompt_structure} illustrates the formal prompt structure.



\begin{itemize}[leftmargin=1em, noitemsep, topsep=1pt]
    \item \textbf{Objective/Task:} Defines the primary task for the LLM, such as generating PoC malware or its deception orchestration code. This directs the model toward producing outputs aligned with the intended goal.
    \item \textbf{Output Format:} Specifies structural and syntactic constraints, including programming language requirements (e.g., C++), library preferences, and function definitions. These specifications drive LLMs to generate executable and compatible codes with the deployment environment.
    \item \textbf{Context:} Provides any supplemental, user-supplied information that may improve the model’s response, such as malware analysis notes, logs, or forensic reports. Knowledge from the ORCAGen KB is not manually added here; instead, relevant entries are automatically retrieved and injected during inference through the RAG pipeline. This separation ensures that context is both flexible for user needs and consistently grounded in verified KB content.
    \item \textbf{Example:} Provides code snippets or minimal working examples that guide the LLM's output to syntactically valid and functional. Example helps LLMs generate more precise and reliable output with reduced risk of hallucination or misunderstanding.
\end{itemize}

\textbf{Prompt Refinement:} If the initial prompt fails to provide functional results, ORCAGen engages in a sequence of iterative refinement prompts. These are targeted follow-up prompts that inject error feedback, highlight missing functionality, or reinforce formatting requirements. This iterative process progressively narrows the model’s output space until runnable PoCs and valid orchestration code are produced. For instance, if the initial PoC output lacks DLL injection logic, the refinement prompt explicitly requests correction, leading the model to regenerate only the missing functionality while preserving previously valid components. This iterative mechanism both improves reliability and provides a measurable indicator of how different LLMs handle complex, domain-specific tasks.

\textbf{Operational Role of the Prompt Template:} The template is executed twice during the workflow: once for generating PoC malware and again for producing deception orchestration code. In both cases, the RAG component automatically injects relevant knowledge from the KB into the prompt at inference time, while users may optionally add their own supplemental context. This structured design ensures that outputs remain context-aware, executable, and scalable across diverse malware families and deception objectives.

\subsection{Code Generation}
The code generation module serves as the core engine of ORCAGen during the offline playbook construction phase. It automatically generates both malware proof-of-concept (PoC) samples and their corresponding deception orchestration code using structured prompts and retrieval-augmented generation (RAG). The goal is to produce behaviorally accurate malware simulations and context-aware defense logic that can be tested before being added to the runtime playbook. This allows ORCAGen to support realistic threat modeling and targeted deception design without requiring live malware during playbook construction.


\subsubsection{Proof-of-Concept (PoC) Code Generation}
The PoC generation component produces representative malware code for a selected threat category, such as keyloggers, information stealers, or ransomware. Its objective is to emulate adversarial behaviors that can later be used to validate deception-based defenses. Once a malware family is selected, ORCAGen queries the RAG-enabled knowledge base to retrieve relevant techniques and behavioral traits. These retrieved entries are embedded into a structured prompt and passed to the Large Language Model (LLM). The LLM combines the retrieved threat intelligence with the template constraints to synthesize PoC malware that reflects real-world techniques. The generated PoC code acts as a controlled and testable instance of the selected malware behavior without requiring access to live threat samples. Once generated, the PoC is evaluated in a controlled environment to confirm that it reproduces the intended behavior. It is also passed to the orchestration code generation module, where it helps guide the creation of corresponding deception logic.
 

\subsubsection{Orchestration Code Generation}
The orchestration code generation module creates active defense mechanisms designed to deceive, disrupt, or neutralize the behavior of a given malware instance. This stage is closely integrated with PoC generation. Once the PoC malware is created, it is combined with relevant active defense strategies retrieved from the RAG-enabled knowledge base. A structured prompt is then passed to the LLM along with the PoC code and the corresponding defense strategies to generate deception-oriented orchestration code. The generated orchestration code is not directly deployed in a live environment. Instead, it is first forwarded to the deployment and testing module, where it is compiled, reviewed, and validated against the emulated malware behavior. Depending on the retrieved active defense strategies, ORCAGen can generate multiple orchestration variants, each corresponding to a specific defensive approach identified in Section~\ref{kb}. Only validated orchestration logic is later included in the deployable deception playbook, implemented as a Super DLL for runtime enforcement.

\begin{figure*}
    \centering
    {\includegraphics[width=0.49\textwidth]{images/poc.pdf}} 
    {\includegraphics[width=0.49\textwidth]{images/orchestration.pdf}} 
    \vspace{-0.2cm}
    \caption{Functionality Validation: (a) PoC Execution Rate, (b) Orchestration Code Execution Rate}
    \vspace{-0.3cm}
    \label{fig:functionality_validation}
\end{figure*}

\subsection{Deployment and Testing}
The deployment and testing phase validates whether the generated deception strategies function effectively before they are added to the runtime playbook. After the PoC malware and its corresponding orchestration code are generated, the PoC is first executed in a controlled environment to confirm that it reproduces the intended malicious behavior, such as credential theft, keystroke logging, file scanning, or file encryption. Once the behavior is confirmed, the orchestration code is compiled and deployed alongside the PoC to assess whether it can deceive, delay, redirect, or neutralize the malicious behavior without exposing the presence of the defense. During this validation stage, interactions between the PoC malware and the generated deception logic are monitored through execution traces, forensic logs, and observed behavior changes. The outcomes are measured using quantitative metrics, including success rate, false positives, and false negatives, along with qualitative observations of adversarial disruption. These results provide the basis for determining whether a generated deception strategy is reliable enough to be included in the final playbook. Only deception strategies that function correctly and pass validation are compiled into a reusable deception playbook, implemented as a Super DLL. This completes the offline generation and validation phase. The validated playbook is then used in the runtime testing phase to evaluate ORCAGen against real-world malware samples collected from public sources.

% \subsection{Testing Phase}
\subsection{Runtime Enforcement Phase}
The runtime enforcement phase evaluates the runtime effectiveness of the validated deception playbook. In this phase, malware samples collected from public sources, such as GitHub, Any.run, VirusTotal are executed in a controlled and instrumented environment. The pre-validated Super DLL is injected into the target process. Once injected, the Super DLL acts as the runtime enforcement module. It monitors malware-relevant API calls, file operations, credential-access attempts, and other behavioral indicators, then triggers the corresponding deception response from the playbook. The system records forensic logs and behavioral changes to determine whether the deployed deception strategy successfully altered, delayed, or suppressed the malware's objective. This phase evaluates the runtime behavior of the playbook, not live LLM inference, since all deception logic has already been generated and validated offline.
